Clarabel: An interior-point solver for conic programs with quadratic objectives

We present a general-purpose interior-point solver for convex optimization problems with conic constraints. Our method is based on a homogeneous embedding method originally developed for general monotone complementarity problems and more recently applied to operator splitting methods, and here specialized to an interior-point method for problems with quadratic objectives. We allow for a variety of standard symmetric and non-symmetric cones, and provide support for chordal decomposition methods in the case of semidefinite cones. We describe the implementation of this method in the open-source solver Clarabel, and provide a detailed numerical evaluation of its performance versus several state-of-the-art solvers on a wide range of standard benchmarks problems. Clarabel is faster and more robust than competing commercial and open-source solvers across a range of test sets, with a particularly large performance advantage for problems with quadratic objectives. Clarabel is currently distributed as a standard solver for the Python CVXPY optimization suite.

==> tables/bench_cblib_pow_detail_table.tex <==
\scriptsize
\begin{longtable}{lcccc||ccc||ccc||}
\caption{\detailtablecaption}
\\
 & &  & & & \multicolumn{3}{c||}{\underline{iterations}}& \multicolumn{3}{c||}{\underline{time per iteration(s)}}& \multicolumn{3}{c||}{\underline{total time (s)}}\\[2ex] 
Problem & vars. & cons. & nnz(A) & nnz(P)  & ClarabelRs & Mosek & ClarabelRs & Mosek & ClarabelRs & Mosek\\[1ex]
\hline
\endhead
\sc{HMCR\_n20\_m400} & 3223 & 2022 & 13239 & 0 &   19 &  \winner  16 &  \winner  0.00236 &   0.00681 &  \winner  0.0448 &   0.109\\ 
\sc{HMCR\_n100\_m400} & 3303 & 2102 & 45315 & 0 &   15 &  \winner  13 &  \winner  0.00698 &   0.00897 &  \winner  0.105 &   0.117\\ 
\sc{HMCR\_n20\_m800} & 6423 & 4022 & 26412 & 0 &   - &  \winner  20 &   - &  \winner  0.0129 &   - &  \winner  0.257\\ 
\sc{HMCR\_n100\_m800} & 6503 & 4102 & 90323 & 0 &   - &  \winner  19 &   - &  \winner  0.0179 &   - &  \winner  0.339\\ 
\sc{HMCR\_n20\_m1200} & 9623 & 6022 & 39575 & 0 &   - &  \winner  27 &   - &  \winner  0.0186 &   - &  \winner  0.503\\ 
\sc{HMCR\_n20\_m1600} & 12823 & 8022 & 52730 & 0 &   - &  \winner  24 &   - &  \winner  0.025 &   - &  \winner  0.599\\ 
\sc{HMCR\_n20\_m2000} & 16023 & 10022 & 65873 & 0 &   - &  \winner  24 &   - &  \winner  0.0308 &   - &  \winner  0.738\\ 
\end{longtable}


==> tables/bench_cblib_pow_sgm.tex <==
\begin{tabular}{llccc}
  \hline
   &  & \textbf{ClarabelRs} & \textbf{Clarabel} & \textbf{Mosek} \\\hline
  Shifted GM & Full Acc. & 163.24 & 163.52 & 1.0 \\
   & Low Acc. & 163.24 & 163.52 & 1.0 \\
  Failure Rate (\%) & Full Acc. & 71.4 & 71.4 & 0.0 \\
   & Low Acc. & 71.4 & 71.4 & 0.0 \\\hline
\end{tabular}


==> tables/bench_cblib_socp_sgm.tex <==
\begin{tabular}{llcccc}
  \hline
   &  & \textbf{ClarabelRs} & \textbf{Clarabel} & \textbf{ECOS} & \textbf{Mosek} \\\hline
  Shifted GM & Full Acc. & 1.0 & 1.11 & 3.39 & 1.27 \\
   & Low Acc. & 1.0 & 1.22 & 3.89 & 4.05 \\
  Failure Rate (\%) & Full Acc. & 10.5 & 10.5 & 26.3 & 10.5 \\
   & Low Acc. & 0.0 & 0.0 & 10.5 & 10.5 \\\hline
\end{tabular}


==> tables/bench_dummy_detail_table.tex <==
\scriptsize
\begin{longtable}{lcccc||ccc||ccc||ccc||}
\caption{\detailtablecaption}
\\
 & &  & & & \multicolumn{3}{c||}{\underline{iterations}}& \multicolumn{3}{c||}{\underline{time per iteration(s)}}& \multicolumn{3}{c||}{\underline{total time (s)}}\\[2ex] 
Problem & vars. & cons. & nnz(A) & nnz(P)  & ClarabelRs & ECOS & Mosek & ClarabelRs & ECOS & Mosek & ClarabelRs & ECOS & Mosek\\[1ex]
\hline
\endhead
\sc{lp} & 1 & 1 & 1 & 0 &   4 &   4 &  \winner  0 &   4.69e-06 &   3.24e-06 &  \winner     0 &   1.87e-05 &  \winner  1.3e-05 &   0.0023\\ 
\sc{qp} & 1 & 1 & 1 & 1 &  \winner  6 &   8 &   7 &   5.34e-06 &  \winner  3.62e-06 &   2.99e-05 &   3.2e-05 &  \winner  2.9e-05 &   0.000209\\ 
\sc{expcone} & 3 & 3 & 3 & 3 &   6 &   14 &  \winner  3 &   7.86e-06 &  \winner  7.77e-06 &   9.04e-05 &  \winner  4.72e-05 &   0.000109 &   0.000271\\ 
\sc{powcone} & 3 & 3 & 3 & 3 &   14 &   - &  \winner  12 &  \winner  5.34e-06 &   - &   2.19e-05 &  \winner  7.48e-05 &   - &   0.000263\\ 
\sc{socp} & 3 & 3 & 3 & 2 &   12 &  \winner  11 &   13 &   6.53e-06 &  \winner  6.41e-06 &   2.55e-05 &   7.84e-05 &  \winner  7.05e-05 &   0.000332\\ 
\sc{sdpcone} & 4 & 4 & 5 & 6 &  \winner  5 &   - &   6 &  \winner  1.6e-05 &   - &   4.83e-05 &  \winner  7.98e-05 &   - &   0.00029\\ 
\sc{mixed} & 9 & 4 & 10 & 6 &  \winner  8 &   - &  \winner  8 &  \winner  2.41e-05 &   - &   3.8e-05 &  \winner  0.000193 &   - &   0.000304\\ 
\end{longtable}


==> tables/bench_dummy_sgm.tex <==
\begin{tabular}{llcccccccccc}
  \hline
   &  & \textbf{ClarabelRs} & \textbf{Clarabel} & \textbf{ECOS} & \textbf{Gurobi} & \textbf{HiGHS} & \textbf{Hypatia} & \textbf{Mosek} & \textbf{OSQP} & \textbf{SCS} & \textbf{Tulip} \\\hline
  Shifted GM & Full Acc. & 2.13 & 5.41 & 2.99559e5 & 7.12785e5 & 1.64688e6 & 35844.4 & 16.12 & 1.6465e6 & 1.0 & 4.61034e6 \\
   & Low Acc. & 2.13 & 5.41 & 2.99559e5 & 7.12785e5 & 1.64688e6 & 32.22 & 16.12 & 1.6465e6 & 1.0 & 4.61034e6 \\
  Failure Rate (\%) & Full Acc. & 0.0 & 0.0 & 42.9 & 57.1 & 71.4 & 14.3 & 0.0 & 71.4 & 0.0 & 85.7 \\
   & Low Acc. & 0.0 & 0.0 & 42.9 & 57.1 & 71.4 & 0.0 & 0.0 & 71.4 & 0.0 & 85.7 \\\hline
\end{tabular}


==> tables/bench_lp_sgm.tex <==
\begin{tabular}{llcccccc}
  \hline
   &  & \textbf{ClarabelRs} & \textbf{Clarabel} & \textbf{ECOS} & \textbf{Gurobi} & \textbf{HiGHS} & \textbf{Mosek} \\\hline
  Shifted GM & Full Acc. & 1.47 & 1.44 & 3.93 & 3.01 & 5.7 & 1.0 \\
   & Low Acc. & 1.47 & 1.44 & 1.7 & 3.01 & 5.7 & 1.0 \\
  Failure Rate (\%) & Full Acc. & 0.0 & 0.0 & 7.1 & 0.0 & 7.1 & 0.0 \\
   & Low Acc. & 0.0 & 0.0 & 0.0 & 0.0 & 7.1 & 0.0 \\\hline
\end{tabular}


==> tables/bench_maros_shifted_detail_table.tex <==
\scriptsize
\begin{longtable}{lcccc||ccc||ccc||ccc||}
\caption{\detailtablecaption}
\\
 & &  & & & \multicolumn{3}{c||}{\underline{iterations}}& \multicolumn{3}{c||}{\underline{time per iteration(s)}}& \multicolumn{3}{c||}{\underline{total time (s)}}\\[2ex] 
Problem & vars. & cons. & nnz(A) & nnz(P)  & ClarabelRs & ECOS & Mosek & ClarabelRs & ECOS & Mosek & ClarabelRs & ECOS & Mosek\\[1ex]
\hline
\endhead
\sc{TAME} & 3 & 2 & 4 & 3 &   5 &   6 &  \winner  4 &   1.59e-05 &  \winner  6.61e-06 &   0.000137 &   7.96e-05 &  \winner  3.96e-05 &   0.000548\\ 
\sc{HS21} & 5 & 2 & 6 & 2 &  \winner  9 &   11 &   11 &  \winner  4.98e-06 &   5.35e-06 &   0.000107 &  \winner  4.48e-05 &   5.88e-05 &   0.00118\\ 
\sc{HS35} & 4 & 3 & 6 & 5 &  \winner  7 &   9 &   9 &   8.92e-06 &  \winner  6.4e-06 &   0.000109 &   6.25e-05 &  \winner  5.76e-05 &   0.000983\\ 
\sc{HS35MOD} & 4 & 3 & 6 & 5 &  \winner  12 &   15 &   14 &  \winner  4.97e-06 &   6.39e-06 &   0.000104 &  \winner  5.96e-05 &   9.58e-05 &   0.00145\\ 
\sc{QPTEST} & 5 & 2 & 7 & 3 &  \winner  8 &   9 &  \winner  8 &   1.5e-05 &  \winner  6.32e-06 &   0.000136 &   0.00012 &  \winner  5.69e-05 &   0.00109\\ 
\sc{HS51} & 3 & 5 & 7 & 7 &  \winner  0 &   9 &   9 &  \winner     0 &   9.16e-06 &   0.000106 &  \winner  4.69e-05 &   8.24e-05 &   0.000955\\ 
\sc{HS52} & 3 & 5 & 7 & 7 &  \winner  0 &   7 &   5 &  \winner     0 &   9.54e-06 &   0.000133 &  \winner  4.8e-05 &   6.68e-05 &   0.000663\\ 
\sc{ZECEVIC2} & 6 & 2 & 8 & 2 &   8 &   8 &  \winner  7 &   6.97e-06 &  \winner  6.94e-06 &   0.000125 &   5.58e-05 &  \winner  5.55e-05 &   0.000878\\ 
\sc{HS268} & 5 & 5 & 25 & 15 &  \winner  12 &   17 &   - &  \winner  6.82e-06 &   9.66e-06 &   - &  \winner  8.18e-05 &   0.000164 &   -\\ 
\sc{S268} & 5 & 5 & 25 & 15 &  \winner  12 &   17 &   - &  \winner  6.54e-06 &   1.12e-05 &   - &  \winner  7.85e-05 &   0.000191 &   -\\ 
\sc{HS76} & 7 & 4 & 14 & 6 &  \winner  6 &   9 &   8 &  \winner  9.08e-06 &   9.25e-06 &   0.000119 &  \winner  5.45e-05 &   8.32e-05 &   0.00095\\ 
\sc{GENHS28} & 8 & 10 & 24 & 19 &  \winner  0 &   10 &   6 &  \winner     0 &   1.17e-05 &   0.000164 &  \winner  3.84e-05 &   0.000117 &   0.000981\\ 
\sc{HS53} & 13 & 5 & 17 & 7 &  \winner  6 &   15 &   7 &  \winner  9.32e-06 &   9.37e-06 &   0.000141 &  \winner  5.59e-05 &   0.000141 &   0.000985\\ 
\sc{LOTSCHD} & 19 & 12 & 66 & 12 &  \winner  9 &   18 &   17 &   3.42e-05 &  \winner  1.88e-05 &   0.000168 &  \winner  0.000307 &   0.000338 &   0.00286\\ 
\sc{HS118} & 59 & 15 & 93 & 15 &  \winner  10 &   15 &  \winner  10 &  \winner  1.75e-05 &   2.39e-05 &   0.00015 &  \winner  0.000175 &   0.000359 &   0.0015\\ 
\sc{QAFIRO} & 59 & 32 & 115 & 35 &   15 &   15 &  \winner  14 &  \winner  2.09e-05 &   3.43e-05 &   0.000208 &  \winner  0.000314 &   0.000514 &   0.00291\\ 
\sc{DPKLO1} & 77 & 133 & 1575 & 133 &  \winner  0 &   14 &   7 &  \winner     0 &   0.000331 &   0.00176 &  \winner  0.000984 &   0.00463 &   0.0123\\ 
\sc{DUAL4} & 151 & 75 & 225 & 2799 &  \winner  12 &  \winner  12 &   14 &  \winner  0.000317 &   0.000467 &   0.000537 &  \winner  0.00381 &   0.0056 &   0.00751\\ 
\sc{QPCBLEND} & 157 & 83 & 574 & 83 &   17 &   18 &  \winner  15 &   0.000141 &  \winner  0.000133 &   0.00105 &   0.00239 &  \winner  0.00239 &   0.0158\\ 
\sc{DUALC1} & 233 & 9 & 1953 & 45 &  \winner  12 &   24 &   - &   0.00019 &  \winner  0.000134 &   - &  \winner  0.00228 &   0.00322 &   -\\ 
\sc{DUALC2} & 243 & 7 & 1617 & 28 &  \winner  11 &   21 &   - &  \winner  9.97e-05 &   0.000104 &   - &  \winner  0.0011 &   0.00218 &   -\\ 
\sc{QADLITTL} & 153 & 97 & 480 & 167 &  \winner  14 &   28 &   - &   0.000142 &  \winner  0.000118 &   - &  \winner  0.00199 &   0.00331 &   -\\ 
\sc{QSHARE2B} & 175 & 79 & 773 & 124 &  \winner  15 &   26 &   - &   0.000224 &  \winner  0.00021 &   - &  \winner  0.00336 &   0.00547 &   -\\ 
\sc{DUAL1} & 171 & 85 & 255 & 3558 &   12 &   15 &  \winner  11 &  \winner  0.000303 &   0.000427 &   0.000727 &  \winner  0.00363 &   0.0064 &   0.008\\ 
\sc{DUAL2} & 193 & 96 & 288 & 4508 &  \winner  11 &   15 &   13 &  \winner  0.000392 &   0.000563 &   0.000811 &  \winner  0.00431 &   0.00845 &   0.0105\\ 
\sc{DUALC5} & 294 & 8 & 2240 & 36 &  \winner  10 &   17 &   15 &  \winner  0.000136 &   0.000202 &   0.000192 &  \winner  0.00136 &   0.00343 &   0.00287\\ 
\sc{CVXQP2\_S} & 225 & 100 & 274 & 386 &  \winner  10 &   21 &   - &  \winner  0.00011 &   0.000202 &   - &  \winner  0.0011 &   0.00424 &   -\\ 
\sc{DUAL3} & 223 & 111 & 333 & 6108 &  \winner  12 &   19 &  \winner  12 &  \winner  0.000677 &   0.000804 &   0.00255 &  \winner  0.00812 &   0.0153 &   0.0306\\ 
\sc{CVXQP1\_S} & 250 & 100 & 348 & 386 &  \winner  9 &   19 &   - &  \winner  0.00019 &   0.000235 &   - &  \winner  0.00171 &   0.00446 &   -\\ 
\sc{CVXQP3\_S} & 275 & 100 & 422 & 386 &  \winner  11 &   22 &   - &  \winner  0.000173 &   0.000241 &   - &  \winner  0.0019 &   0.00531 &   -\\ 
\sc{QSCAGR7} & 269 & 140 & 560 & 157 &  \winner  14 &   40 &   - &  \winner  0.000105 &   0.000154 &   - &  \winner  0.00147 &   0.00616 &   -\\ 
\sc{PRIMAL1} & 86 & 325 & 5816 & 325 &  \winner  10 &   20 &  \winner  10 &   0.000983 &  \winner  0.000858 &   0.00187 &  \winner  0.00983 &   0.0172 &   0.0187\\ 
\sc{PRIMALC1} & 227 & 230 & 2975 & 230 &   - &   - &  \winner  15 &   - &   - &  \winner  0.00224 &   - &   - &  \winner  0.0336\\ 
\sc{PRIMALC2} & 237 & 231 & 2077 & 231 &   - &   - &  \winner  15 &   - &   - &  \winner  0.00229 &   - &   - &  \winner  0.0344\\ 
\sc{QRECIPE} & 340 & 180 & 912 & 210 &  \winner  18 &   22 &   25 &  \winner  0.000148 &   0.000203 &   0.00269 &  \winner  0.00266 &   0.00448 &   0.0672\\ 
\sc{QPCBOEI2} & 382 & 143 & 1480 & 143 &  \winner  20 &   - &   - &  \winner  0.000259 &   - &   - &  \winner  0.00518 &   - &   -\\ 
\sc{DUALC8} & 519 & 8 & 4040 & 36 &  \winner  9 &   27 &   - &   0.000356 &  \winner  0.000291 &   - &  \winner  0.0032 &   0.00786 &   -\\ 
\sc{QSHARE1B} & 342 & 225 & 1376 & 246 &  \winner  19 &   - &   - &  \winner  0.000253 &   - &   - &  \winner  0.0048 &   - &   -\\ 
\sc{PRIMALC5} & 286 & 287 & 2574 & 287 &  \winner  15 &   18 &   - &  \winner  0.000186 &   0.000316 &   - &  \winner  0.00279 &   0.00569 &   -\\ 
\sc{VALUES} & 405 & 202 & 606 & 3822 &  \winner  12 &   16 &   16 &  \winner  0.000337 &   0.00053 &   0.00596 &  \winner  0.00405 &   0.00848 &   0.0953\\ 
\sc{QSC205} & 408 & 203 & 754 & 213 &  \winner  20 &   29 &   23 &  \winner  0.00013 &   0.000181 &   0.00222 &  \winner  0.00259 &   0.00524 &   0.0512\\ 
\sc{QBEACONF} & 435 & 262 & 3637 & 271 &  \winner  16 &   27 &   24 &  \winner  0.000465 &   0.00068 &   0.00469 &  \winner  0.00743 &   0.0184 &   0.112\\ 
\sc{QBRANDY} & 469 & 249 & 2397 & 298 &  \winner  15 &   31 &   24 &  \winner  0.000479 &   0.00054 &   0.0051 &  \winner  0.00718 &   0.0167 &   0.123\\ 
\sc{PRIMAL2} & 97 & 649 & 8043 & 649 &  \winner  8 &   16 &  \winner  8 &  \winner  0.00123 &   0.00145 &   0.00315 &  \winner  0.00982 &   0.0232 &   0.0252\\ 
\sc{QE226} & 505 & 282 & 2860 & 1179 &  \winner  18 &   24 &   24 &  \winner  0.000592 &   0.00106 &   0.00341 &  \winner  0.0107 &   0.0255 &   0.0819\\ 
\sc{PRIMAL3} & 112 & 745 & 21548 & 745 &  \winner  9 &   18 &   10 &   0.00352 &  \winner  0.00304 &   0.00685 &  \winner  0.0317 &   0.0547 &   0.0685\\ 
\sc{QBORE3D} & 559 & 315 & 1755 & 365 &  \winner  19 &   27 &   - &  \winner  0.000309 &   0.000521 &   - &  \winner  0.00588 &   0.0141 &   -\\ 
\sc{KSIP} & 1001 & 20 & 19898 & 20 &   14 &   20 &  \winner  12 &   0.0011 &   0.00117 &  \winner  0.000906 &   0.0153 &   0.0235 &  \winner  0.0109\\ 
\sc{QGROW7} & 721 & 301 & 3193 & 628 &  \winner  26 &   42 &   - &  \winner  0.000417 &   0.000802 &   - &  \winner  0.0108 &   0.0337 &   -\\ 
\sc{QFORPLAN} & 604 & 421 & 5006 & 967 &  \winner  18 &   - &   - &  \winner  0.000749 &   - &   - &  \winner  0.0135 &   - &   -\\ 
\sc{PRIMALC8} & 511 & 520 & 4663 & 520 &  \winner  21 &   - &   - &  \winner  0.00038 &   - &   - &  \winner  0.00798 &   - &   -\\ 
\sc{QCAPRI} & 741 & 353 & 2237 & 1191 &  \winner  31 &   - &   - &  \winner  0.000531 &   - &   - &  \winner  0.0164 &   - &   -\\ 
\sc{QSCORPIO} & 746 & 358 & 1784 & 376 &  \winner  11 &   15 &   16 &  \winner  0.000456 &   0.000625 &   0.00677 &  \winner  0.00502 &   0.00938 &   0.108\\ 
\sc{QSCFXM1} & 787 & 457 & 3046 & 1134 &  \winner  23 &   - &   - &  \winner  0.00058 &   - &   - &  \winner  0.0133 &   - &   -\\ 
\sc{QBANDM} & 777 & 472 & 2966 & 488 &  \winner  20 &   36 &   27 &  \winner  0.00049 &   0.000823 &   0.00747 &  \winner  0.0098 &   0.0296 &   0.202\\ 
\sc{QSCTAP1} & 780 & 480 & 2172 & 597 &  \winner  23 &   31 &   31 &  \winner  0.000339 &   0.000684 &   0.00569 &  \winner  0.00779 &   0.0212 &   0.176\\ 
\sc{QPCSTAIR} & 823 & 467 & 4323 & 467 &  \winner  22 &   - &   - &  \winner  0.000875 &   - &   - &  \winner  0.0192 &   - &   -\\ 
\sc{QPCBOEI1} & 980 & 384 & 4359 & 384 &  \winner  17 &   42 &   - &  \winner  0.000731 &   0.000996 &   - &  \winner  0.0124 &   0.0418 &   -\\ 
\sc{QSCAGR25} & 971 & 500 & 2054 & 600 &  \winner  18 &   - &   - &  \winner  0.000319 &   - &   - &  \winner  0.00573 &   - &   -\\ 
\sc{PRIMAL4} & 76 & 1489 & 16032 & 1489 &  \winner  10 &   21 &   13 &  \winner  0.0026 &   0.00305 &   0.00685 &  \winner  0.026 &   0.0641 &   0.089\\ 
\sc{QSCSD1} & 837 & 760 & 3148 & 1451 &  \winner  12 &   16 &   16 &  \winner  0.000479 &   0.000851 &   0.00724 &  \winner  0.00575 &   0.0136 &   0.116\\ 
\sc{QETAMACR} & 1223 & 688 & 3232 & 4757 &  \winner  20 &   33 &   - &  \winner  0.00425 &   0.00477 &   - &  \winner  0.085 &   0.157 &   -\\ 
\sc{QGROW15} & 1545 & 645 & 6865 & 1107 &  \winner  28 &   43 &   - &  \winner  0.000772 &   0.00142 &   - &  \winner  0.0216 &   0.0611 &   -\\ 
\sc{QFFFFF80} & 1378 & 854 & 7081 & 2492 &  \winner  22 &   - &   - &  \winner  0.00221 &   - &   - &  \winner  0.0486 &   - &   -\\ 
\sc{MOSARQP2} & 1500 & 900 & 3830 & 945 &  \winner  10 &   22 &   18 &  \winner  0.00122 &   0.00184 &   0.0106 &  \winner  0.0122 &   0.0405 &   0.191\\ 
\sc{GOULDQP2} & 1747 & 699 & 2445 & 1047 &  \winner  7 &   19 &   15 &  \winner  0.000533 &   0.000895 &   0.00888 &  \winner  0.00373 &   0.017 &   0.133\\ 
\sc{GOULDQP3} & 1747 & 699 & 2445 & 1396 &  \winner  7 &   25 &   - &  \winner  0.000562 &   0.00105 &   - &  \winner  0.00393 &   0.0262 &   -\\ 
\sc{QSCFXM2} & 1574 & 914 & 6097 & 1971 &  \winner  27 &   - &   - &  \winner  0.00108 &   - &   - &  \winner  0.0291 &   - &   -\\ 
\sc{QSTANDAT} & 1538 & 1075 & 4210 & 1741 &  \winner  18 &   28 &   21 &  \winner  0.000739 &   0.00106 &   0.0111 &  \winner  0.0133 &   0.0297 &   0.234\\ 
\sc{QSCRS8} & 1659 & 1169 & 4351 & 1257 &  \winner  29 &  \winner  29 &   32 &  \winner  0.000802 &   0.00168 &   0.0104 &  \winner  0.0233 &   0.0487 &   0.332\\ 
\sc{QSCSD6} & 1497 & 1350 & 5666 & 2658 &  \winner  16 &   20 &   21 &  \winner  0.000827 &   0.00176 &   0.0131 &  \winner  0.0132 &   0.0352 &   0.276\\ 
\sc{LASER} & 2000 & 1002 & 6000 & 3231 &  \winner  11 &   31 &   - &  \winner  0.000743 &   0.00125 &   - &  \winner  0.00817 &   0.0389 &   -\\ 
\sc{QGFRDXPN} & 1966 & 1092 & 3727 & 1200 &  \winner  23 &   - &   - &  \winner  0.000682 &   - &   - &  \winner  0.0157 &   - &   -\\ 
\sc{QSEBA} & 2057 & 1028 & 5902 & 1578 &  \winner  21 &   - &   - &  \winner  0.000818 &   - &   - &  \winner  0.0172 &   - &   -\\ 
\sc{QGROW22} & 2266 & 946 & 10078 & 1733 &  \winner  30 &   40 &   - &  \winner  0.00117 &   0.00204 &   - &  \winner  0.0352 &   0.0815 &   -\\ 
\sc{CVXQP2\_M} & 2250 & 1000 & 2749 & 3984 &  \winner  10 &   32 &   - &  \winner  0.00448 &   0.0118 &   - &  \winner  0.0448 &   0.377 &   -\\ 
\sc{QSHIP04S} & 1860 & 1458 & 5810 & 1500 &  \winner  15 &   36 &   - &  \winner  0.000838 &   0.00134 &   - &  \winner  0.0126 &   0.0484 &   -\\ 
\sc{CVXQP1\_M} & 2500 & 1000 & 3498 & 3984 &  \winner  10 &   32 &   - &  \winner  0.00681 &   0.0155 &   - &  \winner  0.0681 &   0.497 &   -\\ 
\sc{QSCFXM3} & 2361 & 1371 & 9148 & 2503 &  \winner  27 &   - &   - &  \winner  0.00163 &   - &   - &  \winner  0.0441 &   - &   -\\ 
\sc{CVXQP3\_M} & 2750 & 1000 & 4247 & 3984 &  \winner  12 &   - &   - &  \winner  0.00805 &   - &   - &  \winner  0.0966 &   - &   -\\ 
\sc{Q25FV47} & 2391 & 1571 & 11971 & 60624 &  \winner  26 &   - &   - &  \winner  0.0117 &   - &   - &  \winner  0.305 &   - &   -\\ 
\sc{QSHELL} & 2428 & 1775 & 5448 & 36160 &  \winner  35 &   - &   - &  \winner  0.00617 &   - &   - &  \winner  0.216 &   - &   -\\ 
\sc{QSHIP04L} & 2520 & 2118 & 8450 & 2160 &  \winner  15 &   36 &   - &  \winner  0.00122 &   0.00192 &   - &  \winner  0.0183 &   0.0693 &   -\\ 
\sc{QSCTAP2} & 2970 & 1880 & 8594 & 2516 &  \winner  15 &   28 &   24 &  \winner  0.00168 &   0.00333 &   0.0257 &  \winner  0.0252 &   0.0931 &   0.618\\ 
\sc{AUG3D} & 1000 & 3873 & 6546 & 3873 &  \winner  0 &   - &   11 &  \winner     0 &   - &   0.02 &  \winner  0.00507 &   - &   0.22\\ 
\sc{AUG3DC} & 1000 & 3873 & 6546 & 3873 &  \winner  0 &   - &   - &  \winner     0 &   - &   - &  \winner  0.00518 &   - &   -\\ 
\sc{QSHIP08S} & 3165 & 2387 & 9501 & 13526 &  \winner  15 &   34 &   - &  \winner  0.00345 &   0.00577 &   - &  \winner  0.0517 &   0.196 &   -\\ 
\sc{QPILOTNO} & 3487 & 2172 & 15569 & 2563 &  \winner  31 &   - &   - &  \winner  0.00562 &   - &   - &  \winner  0.174 &   - &   -\\ 
\sc{MOSARQP1} & 3200 & 2500 & 5922 & 2545 &  \winner  10 &   23 &   24 &  \winner  0.00173 &   0.00322 &   0.0345 &  \winner  0.0173 &   0.074 &   0.828\\ 
\sc{QSCSD8} & 3147 & 2750 & 11334 & 5120 &  \winner  14 &   22 &   23 &  \winner  0.00173 &   0.00426 &   0.025 &  \winner  0.0242 &   0.0938 &   0.575\\ 
\sc{QSCTAP3} & 3960 & 2480 & 11354 & 3341 &  \winner  15 &   31 &   26 &  \winner  0.00219 &   0.00489 &   0.0346 &  \winner  0.0328 &   0.152 &   0.898\\ 
\sc{QSHIP12S} & 3914 & 2763 & 10941 & 19124 &  \winner  15 &   37 &   - &  \winner  0.0037 &   0.00623 &   - &  \winner  0.0555 &   0.23 &   -\\ 
\sc{QSIERRA} & 5279 & 2036 & 11354 & 2097 &  \winner  29 &   53 &   - &  \winner  0.00184 &   0.00296 &   - &  \winner  0.0533 &   0.157 &   -\\ 
\sc{STADAT1} & 5999 & 2001 & 13997 & 2001 &  \winner  22 &   - &   - &  \winner  0.00144 &   - &   - &  \winner  0.0317 &   - &   -\\ 
\sc{STADAT2} & 5999 & 2001 & 13997 & 2001 &   35 &   23 &  \winner  22 &  \winner  0.00191 &   0.00471 &   0.0124 &  \winner  0.0667 &   0.108 &   0.272\\ 
\sc{AUG3DCQP} & 4873 & 3873 & 10419 & 3873 &  \winner  11 &   29 &   - &  \winner  0.00356 &   0.00637 &   - &  \winner  0.0392 &   0.185 &   -\\ 
\sc{AUG3DQP} & 4873 & 3873 & 10419 & 3873 &  \winner  12 &   36 &   21 &  \winner  0.00349 &   0.006 &   0.0381 &  \winner  0.0419 &   0.216 &    0.8\\ 
\sc{QSHIP08L} & 5061 & 4283 & 17085 & 38308 &  \winner  16 &   36 &   - &  \winner  0.0147 &   0.0245 &   - &  \winner  0.235 &   0.881 &   -\\ 
\sc{CONT-050} & 7595 & 2597 & 17199 & 2597 &  \winner  8 &   20 &   15 &  \winner  0.00935 &   0.0108 &   0.0442 &  \winner  0.0748 &   0.216 &   0.662\\ 
\sc{EXDATA} & 7501 & 3000 & 12000 & 1127250 &   18 &   22 &  \winner  16 &   0.513 &   0.825 &  \winner  0.148 &   9.23 &   18.1 &  \winner  2.37\\ 
\sc{QSHIP12L} & 6578 & 5427 & 21597 & 65632 &  \winner  16 &   - &   - &  \winner  0.0219 &   - &   - &  \winner  0.35 &   - &   -\\ 
\sc{STCQP1} & 10246 & 4097 & 21532 & 26603 &  \winner  7 &   - &   - &  \winner  0.0106 &   - &   - &  \winner  0.0743 &   - &   -\\ 
\sc{STCQP2} & 10246 & 4097 & 21532 & 26603 &  \winner  9 &   - &   - &  \winner  0.0228 &   - &   - &  \winner  0.205 &   - &   -\\ 
\sc{STADAT3} & 11999 & 4001 & 27997 & 4001 &   46 &  \winner  23 &   25 &  \winner  0.00342 &   0.00836 &   0.0266 &  \winner  0.157 &   0.192 &   0.664\\ 
\sc{HUES-MOD} & 10002 & 10000 & 30000 & 10000 &  \winner  12 &   - &   - &  \winner  0.0053 &   - &   - &  \winner  0.0636 &   - &   -\\ 
\sc{HUESTIS} & 10002 & 10000 & 30000 & 10000 &  \winner  9 &   - &   - &  \winner  0.01 &   - &   - &  \winner  0.0903 &   - &   -\\ 
\sc{LISWET2} & 10000 & 10002 & 30000 & 10002 &  \winner  18 &   - &   - &  \winner  0.00439 &   - &   - &  \winner  0.0789 &   - &   -\\ 
\sc{LISWET3} & 10000 & 10002 & 30000 & 10002 &  \winner  23 &   - &   - &  \winner  0.00427 &   - &   - &  \winner  0.0982 &   - &   -\\ 
\sc{LISWET4} & 10000 & 10002 & 30000 & 10002 &  \winner  27 &   - &   - &  \winner  0.00412 &   - &   - &  \winner  0.111 &   - &   -\\ 
\sc{LISWET5} & 10000 & 10002 & 30000 & 10002 &  \winner  11 &   - &   - &  \winner  0.00497 &   - &   - &  \winner  0.0547 &   - &   -\\ 
\sc{LISWET6} & 10000 & 10002 & 30000 & 10002 &  \winner  18 &   - &   - &  \winner  0.0044 &   - &   - &  \winner  0.0792 &   - &   -\\ 
\sc{DTOC3} & 10000 & 14999 & 34995 & 14999 &  \winner  0 &   - &   12 &  \winner     0 &   - &   0.0919 &  \winner  0.0143 &   - &    1.1\\ 
\sc{AUG2D} & 10000 & 20200 & 40000 & 20200 &  \winner  0 &   - &   - &  \winner     0 &   - &   - &  \winner  0.0313 &   - &   -\\ 
\sc{AUG2DC} & 10000 & 20200 & 40000 & 20200 &  \winner  0 &   - &   - &  \winner     0 &   - &   - &  \winner  0.0292 &   - &   -\\ 
\sc{CVXQP2\_L} & 22500 & 10000 & 27499 & 39984 &  \winner  10 &   - &   - &  \winner  1.35 &   - &   - &  \winner  13.5 &   - &   -\\ 
\sc{CVXQP1\_L} & 25000 & 10000 & 34998 & 39984 &  \winner  11 &   - &   - &  \winner   2.5 &   - &   - &  \winner  27.5 &   - &   -\\ 
\sc{CVXQP3\_L} & 27500 & 10000 & 42497 & 39984 &  \winner  11 &   - &   - &  \winner  2.65 &   - &   - &  \winner  29.2 &   - &   -\\ 
\sc{CONT-100} & 30195 & 10197 & 69399 & 10197 &  \winner  11 &   26 &   13 &  \winner  0.0733 &   0.0983 &   0.199 &  \winner  0.806 &   2.56 &   2.59\\ 
\sc{CONT-101} & 30492 & 10197 & 69993 & 10197 &  \winner  9 &   24 &   13 &  \winner  0.0638 &   0.122 &   0.172 &  \winner  0.574 &   2.93 &   2.24\\ 
\sc{UBH1} & 24018 & 18009 & 60018 & 18009 &   30 &  \winner  26 &   - &  \winner  0.00908 &   0.0205 &   - &  \winner  0.272 &   0.532 &   -\\ 
\sc{AUG2DCQP} & 30200 & 20200 & 60200 & 20200 &  \winner  12 &   - &   - &  \winner  0.02 &   - &   - &  \winner  0.24 &   - &   -\\ 
\sc{AUG2DQP} & 30200 & 20200 & 60200 & 20200 &  \winner  14 &   - &   - &  \winner  0.0201 &   - &   - &  \winner  0.281 &   - &   -\\ 
\sc{CONT-200} & 120395 & 40397 & 278799 & 40397 &  \winner  12 &   22 &   13 &  \winner  0.497 &   0.72 &   0.948 &  \winner  5.97 &   15.8 &   12.3\\ 
\sc{CONT-201} & 120992 & 40397 & 279993 & 40397 &   23 &   22 &  \winner  14 &  \winner  0.626 &   0.678 &   0.928 &   14.4 &   14.9 &  \winner    13\\ 
\sc{BOYD1} & 93279 & 93261 & 652246 & 93261 &  \winner  35 &   - &   - &  \winner  0.0835 &   - &   - &  \winner  2.92 &   - &   -\\ 
\sc{CONT-300} & 271492 & 90597 & 629993 & 90597 &   - &   - &  \winner  16 &   - &   - &  \winner   2.5 &   - &   - &  \winner    40\\ 
\sc{BOYD2} & 279794 & 93263 & 517047 & 93263 &   - &   - &  \winner  28 &   - &   - &  \winner  1.11 &   - &   - &  \winner  31.2\\ 
\end{longtable}


==> tables/bench_maros_shifted_sgm.tex <==
\begin{tabular}{llccccccc}
  \hline
   &  & \textbf{ClarabelRs} & \textbf{Clarabel} & \textbf{ECOS} & \textbf{Gurobi} & \textbf{HiGHS} & \textbf{Hypatia} & \textbf{Mosek} \\\hline
  Shifted GM & Full Acc. & 1.0 & 1.0 & 7.9 & 1.4 & 3.37 & 24.9 & 24.06 \\
   & Low Acc. & 1.0 & 1.01 & 10.75 & 2.08 & 7.34 & 30.65 & 1.49 \\
  Failure Rate (\%) & Full Acc. & 10.9 & 10.9 & 39.1 & 8.0 & 20.3 & 51.4 & 56.5 \\
   & Low Acc. & 3.6 & 4.3 & 31.2 & 2.9 & 20.3 & 37.0 & 0.0 \\\hline
\end{tabular}


==> tables/bench_opf_sdp_sgm.tex <==
\begin{tabular}{llcccc}
  \hline
   &  & \textbf{ClarabelRs} & \textbf{Clarabel} & \textbf{Mosek} & \textbf{SCS} \\\hline
  Shifted GM & Full Acc. & 1.0 & 1.26 & 13.29 & 1.09 \\
   & Low Acc. & 1.44 & 1.0 & 119.95 & 9.85 \\
  Failure Rate (\%) & Full Acc. & 40.0 & 43.3 & 83.3 & 13.3 \\
   & Low Acc. & 13.3 & 10.0 & 83.3 & 13.3 \\\hline
\end{tabular}


==> tables/bench_pow_sgm.tex <==
\begin{tabular}{llccc}
  \hline
   &  & \textbf{ClarabelRs} & \textbf{Clarabel} & \textbf{Mosek} \\\hline
  Shifted GM & Full Acc. & 3.17 & 2.38 & 1.0 \\
   & Low Acc. & 1.0 & 1.0 & 1.33 \\
  Failure Rate (\%) & Full Acc. & 19.2 & 15.4 & 0.0 \\
   & Low Acc. & 0.0 & 0.0 & 0.0 \\\hline
\end{tabular}


==> tables/bench_qp_detail_table.tex <==
\scriptsize
\begin{longtable}{lcccc||ccc||ccc||ccc||}
 &  &  & & & \multicolumn{3}{c||}{\underline{ClarabelRs}}& \multicolumn{3}{c||}{\underline{ECOS}}& \multicolumn{3}{c||}{\underline{Mosek}}\\[2ex] 
Problem & vars. & cons. & nnz(A) & nnz(P)  & iters. & time/iter(s) & total time & iters. & time/iter(s) & total time & iters. & time/iter(s) & total time\\[1ex]
\hline
\sc{issue\_103} & 7 & 5 & 10 & 15 &   7 &   9.81e-06 &   6.87e-05 &   9 &   9.6e-06 &   8.64e-05 &   9 &   0.000115 &   0.00104\\[0.2ex] 
\sc{huber\_fitting\_n\_10} & 45 & 55 & 90 & 15 &   7 &   2.8e-05 &   0.000196 &   10 &   3.05e-05 &   0.000305 &   8 &   0.000214 &   0.00171\\[0.2ex] 
\sc{portfolio\_optimization\_n\_100} & 111 & 110 & 710 & 110 &   11 &   9.62e-05 &   0.00106 &   14 &   0.000124 &   0.00173 &   10 &   0.000725 &   0.00725\\[0.2ex] 
\sc{huber\_fitting\_n\_100} & 450 & 550 & 2604 & 150 &   7 &   0.000754 &   0.00528 &   17 &   0.00107 &   0.0182 &   11 &   0.00375 &   0.0412\\[0.2ex] 
\sc{svm\_L2\_n\_10} & 1000 & 510 & 2019 & 10 &   8 &   0.000402 &   0.00322 &   12 &   0.000411 &   0.00493 &   13 &   0.00161 &   0.021\\[0.2ex] 
\sc{portfolio\_optimization\_n\_1000} & 1101 & 1100 & 52219 & 1100 &   13 &   0.011 &   0.143 &   19 &   0.00876 &   0.167 &   10 &   0.0148 &   0.148\\[0.2ex] 
\sc{huber\_fitting\_n\_500} & 2250 & 2750 & 50327 & 750 &   9 &   0.0302 &   0.272 &   19 &   0.0296 &   0.563 &   15 &   0.0183 &   0.274\\[0.2ex] 
\sc{huber\_fitting\_n\_1000} & 4500 & 5500 & 195240 & 1500 &   9 &   0.223 &   2.01 &   18 &   0.222 &      4 &   16 &   0.0586 &   0.937\\[0.2ex] 
\sc{portfolio\_optimization\_n\_5000} & 5501 & 5500 & 1259971 & 5500 &   17 &   0.549 &   9.34 &   20 &   0.301 &   6.03 &   12 &   0.513 &   6.15\\[0.2ex] 
\sc{svm\_L2\_n\_100} & 10000 & 5100 & 110718 & 100 &   11 &   0.0483 &   0.531 &   17 &   0.0372 &   0.632 &   17 &   0.0142 &   0.242\\[0.2ex] 
\sc{svm\_L2\_n\_500} & 50000 & 25500 & 2548566 & 500 &   12 &   1.02 &   12.2 &   26 &   1.13 &   29.3 &   20 &   0.235 &   4.71\\[0.2ex] 
\end{longtable}


==> tables/bench_qp_sgm.tex <==
\begin{tabular}{llccccccc}
  \hline
   &  & \textbf{ClarabelRs} & \textbf{Clarabel} & \textbf{ECOS} & \textbf{Gurobi} & \textbf{HiGHS} & \textbf{Hypatia} & \textbf{Mosek} \\\hline
  Shifted GM & Full Acc. & 1.48 & 1.48 & 1.87 & 2.68 & 10.63 & 17.73 & 1.0 \\
   & Low Acc. & 1.48 & 1.48 & 1.87 & 2.68 & 10.63 & 17.73 & 1.0 \\
  Failure Rate (\%) & Full Acc. & 0.0 & 0.0 & 0.0 & 0.0 & 27.3 & 18.2 & 0.0 \\
   & Low Acc. & 0.0 & 0.0 & 0.0 & 0.0 & 27.3 & 18.2 & 0.0 \\\hline
\end{tabular}


==> tables/bench_sdp_sgm.tex <==
\begin{tabular}{llccccc}
  \hline
   &  & \textbf{ClarabelRs} & \textbf{Clarabel} & \textbf{Hypatia} & \textbf{Mosek} & \textbf{SCS} \\\hline
  Shifted GM & Full Acc. & 1.0 & 1.89 & 16323.9 & 1.45485e5 & 1200.25 \\
   & Low Acc. & 1.0 & 1.89 & 1076.78 & 1.45485e5 & 1200.25 \\
  Failure Rate (\%) & Full Acc. & 0.0 & 0.0 & 50.0 & 87.5 & 12.5 \\
   & Low Acc. & 0.0 & 0.0 & 12.5 & 87.5 & 12.5 \\\hline
\end{tabular}


==> tables/bench_socp_detail_table.tex <==
\scriptsize
\begin{longtable}{lcccc||ccc||ccc||ccc||}
\caption{\detailtablecaption}
\\
 & &  & & & \multicolumn{3}{c||}{\underline{iterations}}& \multicolumn{3}{c||}{\underline{time per iteration(s)}}& \multicolumn{3}{c||}{\underline{total time (s)}}\\[2ex] 
Problem & vars. & cons. & nnz(A) & nnz(P)  & ClarabelRs & ECOS & Mosek & ClarabelRs & ECOS & Mosek & ClarabelRs & ECOS & Mosek\\[1ex]
\hline
\endhead
\sc{options\_pricing\_K\_10} & 136 & 106 & 280 & 0 &  \winner  9 &   10 &   - &  \winner  7.94e-05 &   0.00012 &   - &  \winner  0.000714 &   0.0012 &   -\\ 
\sc{options\_pricing\_K\_20} & 136 & 106 & 280 & 0 &  \winner  9 &   10 &   19 &  \winner  7.85e-05 &   0.000126 &   0.000422 &  \winner  0.000707 &   0.00126 &   0.00802\\ 
\sc{options\_pricing\_K\_30} & 136 & 106 & 280 & 0 &   13 &  \winner  12 &   - &  \winner  7.02e-05 &   0.000114 &   - &  \winner  0.000913 &   0.00136 &   -\\ 
\sc{options\_pricing\_K\_35} & 136 & 106 & 280 & 0 &  \winner  13 &   - &   - &  \winner  7.62e-05 &   - &   - &  \winner  0.000991 &   - &   -\\ 
\sc{options\_pricing\_K\_40} & 136 & 106 & 280 & 0 &  \winner  12 &   - &   - &  \winner  7.26e-05 &   - &   - &  \winner  0.000871 &   - &   -\\ 
\sc{options\_pricing\_K\_45} & 136 & 106 & 280 & 0 &  \winner  11 &   - &   - &  \winner  7.25e-05 &   - &   - &  \winner  0.000798 &   - &   -\\ 
\sc{options\_pricing\_K\_5} & 136 & 106 & 280 & 0 &  \winner  9 &   10 &   - &  \winner  8.1e-05 &   0.000114 &   - &  \winner  0.000729 &   0.00114 &   -\\ 
\sc{options\_pricing\_K\_50} & 136 & 106 & 280 & 0 &  \winner  11 &   - &   - &  \winner  7.37e-05 &   - &   - &  \winner  0.000811 &   - &   -\\ 
\sc{lasso} & 820 & 419 & 4038 & 419 &  \winner  19 &   - &   - &  \winner  0.000456 &   - &   - &  \winner  0.00866 &   - &   -\\ 
\end{longtable}


==> tables/bench_socp_sgm.tex <==
\begin{tabular}{llccccc}
  \hline
   &  & \textbf{ClarabelRs} & \textbf{Clarabel} & \textbf{ECOS} & \textbf{Hypatia} & \textbf{Mosek} \\\hline
  Shifted GM & Full Acc. & 1.0 & 1.8 & 13548.0 & 13687.4 & 94209.9 \\
   & Low Acc. & 1.0 & 1.8 & 1517.82 & 1570.04 & 94209.9 \\
  Failure Rate (\%) & Full Acc. & 0.0 & 0.0 & 55.6 & 55.6 & 88.9 \\
   & Low Acc. & 0.0 & 0.0 & 22.2 & 22.2 & 88.9 \\\hline
\end{tabular}

